Reflect-Push Methods Part I: Two Dimensional Techniques

We determine all maximum weight downsets in the product of two chains, where the weight function is a strictly increasing function of the rank. Many discrete isoperimetric problems can be reduced to the maximum weight downset problem. Our results generalize Lindsay's edge-isoperimetric theorem in two dimensions in several directions. They also imply and strengthen (in several directions) a result of Ahlswede and Katona concerning graphs with maximal number of adjacent pairs of edges. We find all optimal shifted graphs in the Ahlswede-Katona problem. Furthermore, the results of Ahlswede-Katona are extended to posets with a rank increasing and rank constant weight function. Our results also strengthen a special case of a recent result by Keough and Radcliffe concerning graphs with the fewest matchings. All of these results are achieved by applications of a key lemma that we call the reflect-push method. This method is geometric and combinatorial. Most of the literature on edge-isoperimetric inequalities focuses on finding a solution, and there are no general methods for finding all possible solutions. Our results give a general approach for finding all compressed solutions for the above edge-isoperimetric problems. By using the Ahlswede-Cai local-global principle, one can conclude that lexicographic solutions are optimal for many cases of higher dimensional isoperimetric problems. With this and our two dimensional results we can prove Lindsay's edge-isoperimetric inequality in any dimension. Furthermore, our results show that lexicographic solutions are the unique solutions for which compression techniques can be applied in this general setting.

==> colors2D.tex <==
%auto-ignore
\newcommand{\typeA}{magenta!65}
\newcommand{\typeB}{blue!75}
\newcommand{\original}{red}
\newcommand{\reflect}{yellow}
\newcommand{\push}{green!70}
\newcommand{\double}{lime!70}


==> colors3D.tex <==
%auto-ignore
\newcommand{\typeA}{magenta!55}
\newcommand{\typeB}{blue!65}


==> settings3D.tex <==
%auto-ignore
\psset{viewpoint=50 40 20 rtp2xyz,Decran=50}
\psset{lightsrc=20 35 45,linewidth=0.5\pslinewidth}

